Robust Structure-based Shape Correspondence

We present a robust method to find region-level correspondences between shapes, which are invariant to changes in geometry and applicable across multiple shape representations. We generate simplified shape graphs by jointly decomposing the shapes, and devise an adapted graph-matching technique, from which we infer correspondences between shape regions. The simplified shape graphs are designed to primarily capture the overall structure of the shapes, without reflecting precise information about the geometry of each region, which enables us to find correspondences between shapes that might have significant geometric differences. Moreover, due to the special care we take to ensure the robustness of each part of our pipeline, our method can find correspondences between shapes with different representations, such as triangular meshes and point clouds. We demonstrate that the region-wise matching that we obtain can be used to find correspondences between feature points, reveal the intrinsic self-similarities of each shape, and even construct point-to-point maps across shapes. Our method is both time and space efficient, leading to a pipeline that is significantly faster than comparable approaches. We demonstrate the performance of our approach through an extensive quantitative and qualitative evaluation on several benchmarks where we achieve comparable or superior performance to existing methods.

==> applications.tex <==
We present two applications for the symmetry aware correspondence between segments. First, we use this correspondence to enhance point-to-point maps between the shapes. For this, we use the functional map framework of Ovsjanikov et al. In~\cite{ovsjanikov12}, the point-to-point maps are improved using large and sparse segments (i.e., the segments do not cover the whole shape). The segments in that work are not symmetric. Naturally, breaking the symmetry of our segments prior to computing the maps can be helpful. However, in this work we aim to show that the matching between symmetric segments, which can be found quickly and in a stable manner, can still greatly improve the point-to-point maps without first resolving the ambiguity. The advantage of using our approach is the use of dense and stable segments: our segments cover the whole shape and are more accurate than the large segments used in~\cite{ovsjanikov12}.

% TODO: Turn this into evaluation section. Have a section for evaluation of the segments comparing to BIM. Then a section for the point to point maps, including the table of results and discussing the fact that WKS is not necessary when using those segments.
% Finally, add the symmetry detection application as another section in the evaluation.

% Also add the timing in this section...

==> fig_gallery.tex <==
\begin{figure*}[t]
\centering

\begin{minipage}{0.9\linewidth}
	\centering

	\begin{minipage}{0.31\linewidth}
	    \centering
	    \includegraphics[width=\linewidth]{images/mesh040_mesh018}
	    %(a)
	\end{minipage}
	\begin{minipage}{0.31\linewidth}
	    \centering
	    \includegraphics[width=\linewidth]{images/david11_david13_10}
	    %(b)
	\end{minipage}
	\begin{minipage}{0.36\linewidth}
	    \centering
	    \includegraphics[width=\linewidth]{images/michael2_victoria23}
	    %(c)
	\end{minipage}
	
	\begin{minipage}{0.31\linewidth}
		\centering
		(a)
	\end{minipage}
	\begin{minipage}{0.31\linewidth}
		\centering
		(b)
	\end{minipage}
	\begin{minipage}{0.36\linewidth}
		\centering
		(c)
	\end{minipage}

	\begin{minipage}{0.25\linewidth}
	    \centering
	    \includegraphics[width=\linewidth]{images/michael4_gorilla14_7}
	    %(d)
	\end{minipage}
	\begin{minipage}{0.36\linewidth}
	    \centering
	    \includegraphics[width=\linewidth]{images/cat3_cat2}
	    %(e)
	\end{minipage}
	\begin{minipage}{0.36\linewidth}
	    \centering
	    \includegraphics[width=\linewidth]{images/arma_281_294}
	    %(f)
	\end{minipage}

	\begin{minipage}{0.25\linewidth}
	    \centering
	    (d)
	\end{minipage}
	\begin{minipage}{0.36\linewidth}
	    \centering
	    (e)
	\end{minipage}
	\begin{minipage}{0.36\linewidth}
	    \centering
	    (f)
	\end{minipage}


	\begin{minipage}{0.32\linewidth}
	    \centering
	    \includegraphics[width=\linewidth]{images/049_004}
	    %(g)
	\end{minipage}
	\begin{minipage}{0.32\linewidth}
	    \centering
	    \includegraphics[width=\linewidth]{images/069_041}
	    %(h)
	\end{minipage}
	\begin{minipage}{0.35\linewidth}
	    \centering
	    \includegraphics[width=\linewidth]{images/029_084}
	    %(i)
	\end{minipage}
	
	\begin{minipage}{0.32\linewidth}
		\centering
		(g)
	\end{minipage}
	\begin{minipage}{0.32\linewidth}
		\centering
		(h)
	\end{minipage}
	\begin{minipage}{0.35\linewidth}
		\centering
		(i)
	\end{minipage}

\end{minipage}

	%\begin{tabular}{@{}c@{\,}c@{\,}c@{}}
%
		%\includegraphics[width=0.33\linewidth]{images/mesh040_mesh018} &
		%\includegraphics[width=0.33\linewidth]{images/david11_david13_10} &
		%\includegraphics[width=0.33\linewidth]{images/michael2_victoria23} \\
		%
		%(a) & (b) & (c) \\
		%
		%\includegraphics[width=0.33\linewidth]{images/michael4_gorilla14_7} &
		%\includegraphics[width=0.33\linewidth]{images/cat3_cat2} &
		%\includegraphics[width=0.33\linewidth]{images/centaur3_centaur0_7} \\
%
		%(d) & (e) & (f) \\
%
	%\end{tabular}

\caption[Symmetry aware correspondence between shapes]{Region-based
  symmetric correspondence between shapes.
\label{fig:symmetry_gallery}}
\vspace{-5mm}
\end{figure*}

